Internal Structure, Not Environment, Shapes Metallicity Gradients in Low-Mass Galaxies from MaNGA

Dwarf and low-mass galaxies are highly sensitive to stellar feedback and gas flows, yet their spatially resolved gas-phase metallicity remains poorly characterised. We measure radial gas-phase metallicity gradients for 382 star-forming low-mass galaxies from MaNGA DR17, spanning $7.2 \leq \log(M_{\star}/M_{\odot}) \leq 9.1$ and $z \leq 0.05$. Spectra are stacked in elliptical radial bins and metallicity is derived from the N2 index. After removing the primary dependence on local stellar mass surface density, we define a residual metallicity $\Delta Z$ to isolate secondary dependencies. Gradients are flat on average (median slope $-0.007$\,dex\,$R_e^{-1}$). The residual gradients correlate most strongly with light concentration ($r = 0.304$, $r^2 = 0.092$, $p < 0.001$) and gas velocity dispersion ($r = 0.204$, $p < 0.001$), though both account for at most 9 per cent of the variance. Large-scale environment shows no significant correlation. The concentration result is robust to measurement uncertainties and persists with a stricter resolution cut, suggesting internal structural properties shape the radial metal distribution in low-mass galaxies.

==> table_master.tex <==
\begin{longtab}
\begin{longtable}{lccccrrrrl}
\caption{\label{tab:master} Key properties 
of the 382 low-mass galaxies in our final 
sample, sorted by stellar mass. The full 
table is available online; the first 50 
entries are shown here. Columns give the 
MaNGA plate-IFU identifier, spectroscopic 
redshift, log stellar mass, effective 
radius, spatial resolution ratio 
$R_{\rm e}/\theta_{\rm PSF}$, metallicity 
gradient slope and its $1\sigma$ 
uncertainty, corrected residual metallicity 
gradient slope and its $1\sigma$ 
uncertainty, and visual classification. 
Galaxies with corrected redshifts 
(Section~\ref{sec:redshift}) may fall 
outside the nominal selection range 
$0.01 \leq z \leq 0.05$.}\\
\hline\hline
\noalign{\smallskip}
PlateIFU & $z$ & $\log M_{\star}$ & 
$R_{\rm e}$ & $R_{\rm e}/\theta_{\rm PSF}$ & 
$\nabla Z$ & $\sigma_{\nabla Z}$ & 
$\nabla\Delta Z$ & $\sigma_{\nabla\Delta Z}$ & 
Class \\
\noalign{\smallskip}
& & ($M_{\odot}$) & (\arcsec) & & 
\multicolumn{2}{c}{(dex\,$R_{\rm e}^{-1}$)} & 
\multicolumn{2}{c}{(dex\,$R_{\rm e}^{-1}$)} & \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endfirsthead
\caption{continued.}\\
\hline\hline
\noalign{\smallskip}
PlateIFU & $z$ & $\log M_{\star}$ & 
$R_{\rm e}$ & $R_{\rm e}/\theta_{\rm PSF}$ & 
$\nabla Z$ & $\sigma_{\nabla Z}$ & 
$\nabla\Delta Z$ & $\sigma_{\nabla\Delta Z}$ & 
Class \\
\noalign{\smallskip}
& & ($M_{\odot}$) & (\arcsec) & & 
\multicolumn{2}{c}{(dex\,$R_{\rm e}^{-1}$)} & 
\multicolumn{2}{c}{(dex\,$R_{\rm e}^{-1}$)} & \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endhead
\noalign{\smallskip}
\hline
\endfoot
\noalign{\smallskip}
\hline
\endlastfoot
\noalign{\smallskip}
9049-6101 & 0.0139 & 7.84 & 7.35 & 2.94 & $-0.094$ & $0.023$ & $-0.052$ & $0.027$ & ISOLATED \\
8981-12705 & 0.0057 & 8.12 & 6.10 & 2.44 & $-0.076$ & $0.013$ & $-0.023$ & $0.016$ & ISOLATED \\
8619-12705 & 0.0116 & 8.27 & 7.87 & 3.15 & $-0.085$ & $0.016$ & $-0.043$ & $0.013$ & DISTURBED \\
9493-12702 & 0.0122 & 8.32 & 7.14 & 2.86 & $-0.081$ & $0.008$ & $-0.037$ & $0.009$ & ISOLATED \\
8546-12702 & 0.0125 & 8.37 & 6.48 & 2.59 & $+0.019$ & $0.012$ & $+0.072$ & $0.014$ & ISOLATED \\
9502-6102 & 0.0173 & 8.39 & 7.59 & 3.03 & $+0.003$ & $0.016$ & $+0.025$ & $0.022$ & ISOLATED \\
8565-6104 & 0.0094 & 8.40 & 4.72 & 1.89 & $+0.087$ & $0.012$ & $+0.138$ & $0.012$ & ISOLATED \\
9093-1902 & 0.0220 & 8.40 & 3.04 & 1.22 & $+0.017$ & $0.012$ & $+0.053$ & $0.015$ & ISOLATED \\
8993-6101 & 0.0196 & 8.42 & 7.48 & 2.99 & $-0.037$ & $0.008$ & $-0.047$ & $0.008$ & ISOLATED \\
8619-12704 & 0.0206 & 8.45 & 5.57 & 2.23 & $-0.032$ & $0.008$ & $+0.005$ & $0.013$ & ISOLATED \\
8719-9101 & 0.0178 & 8.46 & 12.38 & 4.95 & $+0.028$ & $0.050$ & $+0.084$ & $0.047$ & DISTURBED \\
8082-3701 & 0.0213 & 8.46 & 2.87 & 1.15 & $+0.036$ & $0.007$ & $+0.078$ & $0.008$ & DISTURBED \\
8982-12702 & 0.0250 & 8.49 & 6.81 & 2.72 & $-0.095$ & $0.011$ & $-0.066$ & $0.006$ & ISOLATED \\
8552-3701 & 0.0183 & 8.50 & 4.46 & 1.78 & $+0.104$ & $0.015$ & $+0.154$ & $0.018$ & DISTURBED \\
9886-6102 & 0.0219 & 8.54 & 6.62 & 2.65 & $+0.017$ & $0.016$ & $+0.065$ & $0.017$ & ISOLATED \\
8338-1901 & 0.0215 & 8.54 & 3.19 & 1.28 & $+0.106$ & $0.017$ & $+0.157$ & $0.019$ & DISTURBED \\
8657-6104 & 0.0175 & 8.56 & 5.17 & 2.07 & $-0.027$ & $0.010$ & $+0.016$ & $0.009$ & DISTURBED \\
8149-6103 & 0.0221 & 8.56 & 5.36 & 2.14 & $-0.072$ & $0.015$ & $-0.048$ & $0.010$ & DISTURBED \\
11022-12702 & 0.0228 & 8.56 & 6.00 & 2.40 & $+0.089$ & $0.017$ & $+0.124$ & $0.014$ & ISOLATED \\
9494-6102 & 0.0157 & 8.56 & 6.04 & 2.41 & $+0.173$ & $0.033$ & $+0.199$ & $0.038$ & ISOLATED \\
8996-6104 & 0.0214 & 8.57 & 6.62 & 2.65 & $-0.011$ & $0.008$ & $-0.020$ & $0.008$ & ISOLATED \\
9001-12704 & 0.0212 & 8.59 & 8.94 & 3.58 & $-0.030$ & $0.015$ & $+0.010$ & $0.020$ & ISOLATED \\
8447-1901 & 0.0202 & 8.59 & 3.16 & 1.27 & $-0.026$ & $0.005$ & $+0.020$ & $0.004$ & ISOLATED \\
8459-9102 & 0.0170 & 8.59 & 7.75 & 3.10 & $+0.021$ & $0.016$ & $+0.063$ & $0.017$ & ISOLATED \\
8553-12703 & 0.0136 & 8.61 & 12.40 & 4.96 & $+0.198$ & $0.053$ & $+0.241$ & $0.056$ & DISTURBED \\
9886-3701 & 0.0216 & 8.62 & 12.84 & 5.13 & $-0.151$ & $0.091$ & $-0.063$ & $0.098$ & DISTURBED \\
8563-3704 & 0.0192 & 8.63 & 3.79 & 1.52 & $+0.047$ & $0.007$ & $+0.095$ & $0.007$ & ISOLATED \\
8987-6101 & 0.0219 & 8.63 & 5.10 & 2.04 & $-0.069$ & $0.008$ & $-0.048$ & $0.006$ & ISOLATED \\
8241-6101 & 0.0209 & 8.63 & 5.82 & 2.33 & $+0.104$ & $0.038$ & $+0.162$ & $0.040$ & DISTURBED \\
8566-6103 & 0.0103 & 8.64 & 4.69 & 1.88 & $-0.018$ & $0.005$ & $+0.020$ & $0.009$ & ISOLATED \\
8564-1901 & 0.0196 & 8.64 & 3.35 & 1.34 & $+0.044$ & $0.008$ & $+0.079$ & $0.011$ & DISTURBED \\
8439-1901 & 0.0164 & 8.65 & 3.21 & 1.28 & $+0.097$ & $0.007$ & $+0.143$ & $0.006$ & ISOLATED \\
8135-6101 & 0.0109 & 8.65 & 6.84 & 2.74 & $+0.077$ & $0.016$ & $+0.112$ & $0.014$ & DISTURBED \\
8936-6104 & 0.0142 & 8.65 & 6.16 & 2.46 & $+0.094$ & $0.017$ & $+0.158$ & $0.020$ & DISTURBED \\
10517-12704 & 0.0132 & 8.66 & 9.39 & 3.76 & $-0.289$ & $0.132$ & $-0.128$ & $0.107$ & DISTURBED \\
8991-3703 & 0.0191 & 8.66 & 4.41 & 1.77 & $-0.006$ & $0.004$ & $+0.041$ & $0.004$ & ISOLATED \\
10496-12703 & 0.0189 & 8.66 & 12.05 & 4.82 & $-0.068$ & $0.009$ & $-0.045$ & $0.008$ & DISTURBED \\
11977-12704 & 0.0211 & 8.66 & 10.06 & 4.02 & $-0.033$ & $0.015$ & $+0.025$ & $0.022$ & DISTURBED \\
9001-9102 & 0.0214 & 8.66 & 2.64 & 1.05 & $+0.073$ & $0.003$ & $+0.106$ & $0.005$ & ISOLATED \\
8567-6102 & 0.0227 & 8.66 & 3.81 & 1.52 & $+0.013$ & $0.008$ & $+0.041$ & $0.011$ & DISTURBED \\
8552-6101 & 0.0180 & 8.66 & 6.54 & 2.62 & $-0.050$ & $0.010$ & $-0.042$ & $0.005$ & DISTURBED \\
9485-9102 & 0.0188 & 8.67 & 7.91 & 3.16 & $-0.002$ & $0.011$ & $-0.011$ & $0.007$ & DISTURBED \\
8716-12701 & 0.0190 & 8.67 & 7.45 & 2.98 & $-0.009$ & $0.001$ & $-0.015$ & $0.002$ & DISTURBED \\
8987-6103 & 0.0217 & 8.67 & 7.52 & 3.01 & $-0.063$ & $0.007$ & $-0.025$ & $0.011$ & ISOLATED \\
9500-3702 & 0.0216 & 8.68 & 4.60 & 1.84 & $+0.069$ & $0.010$ & $+0.121$ & $0.015$ & DISTURBED \\
8323-12702 & 0.0230 & 8.68 & 8.99 & 3.60 & $+0.207$ & $0.052$ & $+0.250$ & $0.054$ & ISOLATED \\
8551-6101 & 0.0188 & 8.68 & 7.30 & 2.92 & $-0.052$ & $0.008$ & $-0.035$ & $0.005$ & DISTURBED \\
9033-1901 & 0.0185 & 8.69 & 3.37 & 1.35 & $+0.026$ & $0.005$ & $+0.071$ & $0.008$ & ISOLATED \\
10506-12704 & 0.0173 & 8.69 & 6.84 & 2.74 & $+0.034$ & $0.008$ & $+0.072$ & $0.007$ & ISOLATED \\
8257-3704 & 0.0202 & 8.69 & 4.66 & 1.86 & $+0.011$ & $0.016$ & $+0.051$ & $0.011$ & DISTURBED \\
\noalign{\smallskip}
\hline
\end{longtable}
\end{longtab}
